Verification of Hierarchical Artifact Systems

Data-driven workflows, of which IBM's Business Artifacts are a prime exponent, have been successfully deployed in practice, adopted in industrial standards, and have spawned a rich body of research in academia, focused primarily on static analysis. The present work represents a significant advance on the problem of artifact verification, by considering a much richer and more realistic model than in previous work, incorporating core elements of IBM's successful Guard-Stage-Milestone model. In particular, the model features task hierarchy, concurrency, and richer artifact data. It also allows database key and foreign key dependencies, as well as arithmetic constraints. The results show decidability of verification and establish its complexity, making use of novel techniques including a hierarchy of Vector Addition Systems and a variant of quantifier elimination tailored to our context.

==> expressiveness.tex <==
%lock: Victor


\section{Expressive completeness of HLTL-FO} \label{sec:completeness}

We next further motivate the use of the temporal logic HLTL-FO by showing that it is, in a significant sense, 
expressively complete. Moreover, HLTL-FO allows the use of partial-order model-checking techniques, 
thus avoiding the exponential blowup caused by considering all interleavings of concurrent actions of independent tasks. 

We first recall the logic LTL-FO, slightly adapted to our context. For simplicity we assume 
throughout this section that there are no global variables (these can be easily accounted for).
Let $\Gamma = \langle \cala, \Sigma, \Pi \rangle$ be an artifact system where 
$\cala = \langle \calt, \calh, \mathcal{DB}, \Delta \rangle$.
An LTL-FO formula over $\Gamma$ consists of an LTL formula $\varphi$ with propositions $P \cup \Sigma$ 
together with a mapping $f$ associating to each $p \in P$ a condition over $\bar x^T$ for some $T\ \in \calt$
(and we say that $f(p)$ is over $T$) . 
Satisfaction of $\varphi_f$ on 
a run $\rho = \{(\rho_i,\sigma_i)\}_{i \geq 0}$ of $\Gamma$ on database $D$, 
where $\rho_i = (\nu_i, stg_i, D, S_i)$,
is defined as usual, modulo the following:
\begin{itemize}
%\item $active_T$ holds in $(\rho_i,\sigma_i)$ if $stg_i(T) = \emph{active}$
\item $f(p)$ over $T$ holds in $(\rho_i,\sigma_i)$ iff $stg_i(T) = \emph{active}$ and the condition 
$f(p)$ on $\nu_i(\bar x^T)$ holds; 
%\item proposition $S_T$ holds in $(\rho_i,\sigma_i)$ iff $stg_i(T) = \emph{active}$ and $S_T(\nu_i(\bar x^T))$ holds;
\item proposition $\sigma$ in $\Sigma$ holds in $(\rho_i, \sigma_i)$ if $\sigma = \sigma_i$.
\end{itemize}
An {\em isomorphism type} of $\bar x^T$ consists of its isomorphism type with respect to the signature $\mathcal{DB}$ 
together with the truth value of $S_T(\bar x^T)$. 
The information about $(\rho_i,\sigma_i)$ relevant to satisfaction of $\varphi_f$ consists of
$\sigma_i$, the stage of each task (active/inactive), and the isomorphism type of $\nu_i(\bar x^T)$
(for active tasks $T$). 
 
By definition, LTL-FO operates on runs of $\Gamma$ consisting of interleavings of the actions of all tasks.
In particular, this includes all distinct interleavings of independent tasks. Clearly, we are only interested 
in properties that are invariant under such interleavings. This is not only a natural soundness condition, but also
allows more efficient model checking. Indeed, rather than considering all interleavings, it is sufficient to
consider only one representative of all interleavings compatible with the 
dependencies among tasks. This approach is well-known in verification of concurrent systems as 
{\em partial-order model checking} \cite{}.
It is clear that LTL-FO also expresses properties that are {\em not} invariant under interleavings.

We will show that HLTL-FO expresses precisely the LTL-FO properties that are invariant under interleavings.
We first need to make more precise the notion of invariance under interleavings.
Consider an LTL-FO formula $\varphi_f$ over $\Gamma$. Invariance under interleavings is a property of
the propositional formula $\varphi$. Let $P \cup \Sigma$ be the set of propositions of $\varphi$ and let $P_T$
denote the subset of $P$ for which $f(p)$ is a condition over $\bar x^T$. Thus, $\{P_T \mid T \in \calt\}$
is a partition of $P$. 
%For each $T \in \calt$, let $\bar \Sigma_T = \Sigma_T \cup \{\sigma^o_T, \sigma^c_T\} \cup
%\{\sigma^c_{T'} \mid T' \in \emph{child}(T)\}$. Intuitively, $\bar \Sigma_T$ consists of the services that may 
%affect the values of the conditions over $\bar x^T$, so of the propositions in $P_T$. 
%Observe that $\bar \Sigma_T \cap \bar \Sigma_{T'} = \{\sigma_{T'}^c\}$ if $T' \in \emph{child}(T)$.
   
We define the set $\call_\Gamma$ of $\omega$-words associated to $\Gamma$, on which $\varphi$ operates. 
The alphabet, denoted ${\bf A}(\Gamma)$, consists of all triples $(\kappa, stg, \sigma)$ where $\sigma \in \Sigma$, 
$\kappa$ is a truth assignment to the propositions in $P$, and $stg$ is a mapping associating to each $T \in \calt$ 
its stage (active, init, or closed).  
%For each $T \in \calt$, let $\bar \Sigma_T = \Sigma_T \cup \{\sigma_T^o\} \cup \{\sigma_{\bar T}^c \mid \bar T \in \emph{child}(T)\}$.
An $\omega$-word $\{(\kappa_i, stg_i,  \sigma_i)\}_{i \geq 0}$ over ${\bf A}(\Gamma)$ is in $\call_\Gamma$ 
if the following hold:
\begin{itemize}
\item [(i)] for each $i > 0$, if $\sigma_i \in \Sigma^\delta_T$, then
$\kappa_i$ and $\kappa_{i-1}$ agree on all $P_{\bar T}$ where $\bar T \neq T$;
\item [(ii)] the sequence of calls, returns, and internal services obeys the hierarchical structure of $\Gamma$;
\item [(iii)] for each $i > 0$ and $T \in \calt$, $stg_i(T)$ is the stage of $T$ as determined by the sequence
of calls and returns in $\{\sigma_j\}_{j < i}$.
\end{itemize}
The formal definition of $(ii)$ and $(iii)$ mimicks closely the analogous definition for runs of 
artifact systems (omitted).

Consider an $\omega$-word $u = \{(\kappa_i, stg_i, \sigma_i)\}_{i \geq 0}$ in $\call_\Gamma$. 
%We define the projection of $u$ on $T$ as the subsequence $\pi_T(u) = \{(\kappa_{i_j}|_{P_T}, stg_{i_j}(T), \sigma_{i_j})\}_{j \geq 0}$ where $\{\sigma_{i_j} \mid j \geq 0\}$ is the subsequence of $\{\sigma_i \mid i \geq 0\}$ retaining all services 
%in $\bar \Sigma_T$.
We define the partial order $\preceq_u$ on $\{ i \mid i \geq 0\}$ as the reflexive-transitive closure of the
relation consisting of all pairs $(i,j)$ such that $i < j$ and for some $T$, 
$\sigma_i, \sigma_j \in \Sigma^{obs}_T$. 
Observe that $0$ is always the minimum element in $\preceq_u$.
A linearization of $\preceq_u$ is a total order on $\{ i \mid i \geq 0\}$ containing $\preceq_u$.  
One can represent a linearization of $\preceq_u$ as a sequence 
%$\{i_j \mid j \geq 0 i_{j+1} \not\preceq_u i_j\}$.  
$\{i_j \mid j \geq 0\}$ such that $i_n \preceq_u i_m$ implies that $n \leq m$.  
For each such linearization $\alpha$ we define the $\omega$-word 
$u_\alpha  = \{(\bar \kappa_j, \overline{\emph{stg}}_j, \sigma_{i_j})\}_{ j \geq 0}$  
in $\call_\Gamma$ as follows. The stage function is the one determined by the sequence of services.
The functions $\bar \kappa_j$ are defined by induction as follows:
\begin{itemize}
\item $\bar \kappa_{0} = \kappa_0$;
\item if $j >0$ and $\sigma_{i_j} \in \Sigma^\delta_T$ 
then $\bar \kappa_{j}$ agrees with $\bar \kappa_{j-1}$ on all $P_{\bar T}$ where $\bar T \neq T$
and $\bar \kappa_{j}|_{P_T} = \kappa_{i_j}|_{P_T}$.  
\end{itemize}
Intuitively, $u_\alpha$ is obtained from $u$ by commuting actions that are incomparable with respect to $\preceq_u$,
yielding the linearization $\alpha$.

We note that the relation $\preceq_u$ is the analog to our setting of Mazurkiewicz 
traces, used in concurrent systems to capture dependencies among process actions \cite{}.

\begin{definition}
An LTL-FO formula $\varphi_f$ over $\Gamma$ is invariant with respect to interleavings if for every
$u \in \call_\Gamma$ and linearization $\alpha$ of $\preceq_u$ , 
$~~u \models \varphi~~$  iff  $~~u_\alpha \models \varphi$. 
\end{definition}

We can show the following completeness result.

\begin{theorem} \label{thm:complete}
HTL-FO expresses precisely the LTL-FO properties of 
hierarchical transition systems invariant with respect to interleavings.
\end{theorem}

We outline the proof in the remainder of the section.
We first show a useful normal form for LTL formulas. 
Consider the alphabet ${\bf H}(\Gamma) = \{(\kappa, \sigma) \mid (\kappa, stg, \sigma) \in {\bf A}(\Gamma)\}$.
Thus, ${\bf H}(\Gamma)$ is ${\bf A}(\Gamma)$ with the stage information omitted.
Let $\calh(\Gamma) = h(\call(\Gamma))$
where $h((\kappa,stg,\sigma)) = (\kappa, \sigma)$. 
We define local-LTL to be LTL 
using the set of propositions P$\Sigma$ consisting of all pairs $(p,\sigma)$ where $\sigma \in \Sigma$ and 
$p \in P_T$ if $\sigma \in \Sigma_T$, $p \in P_T \cup P_{T_c}$ if $T_c$ is a child of $T$ and 
$\sigma \in \{\sigma^o_{T_c}, \sigma^c_{T_c}\}$, and $p \in P_{T_1}$ if $\sigma = \sigma^o_{T_1}$.
%if $\sigma \in \Sigma_T \cup \{\sigma^o_{T'} \mid T' \in \emph{child}(T)\}$ and
%$p \in P_T \cup P_{T'}$ if $\sigma = \sigma^c_{T'}$ where $T' \in \emph{child}(T)$. 
A proposition
$(p,\sigma)$ holds in $(\bar \kappa,\bar \sigma)$ iff $\bar \sigma = \sigma$ and $\bar \kappa(p)$ is true.    

\begin{lemma} \label{lem:local-ltl}
For each LTL formula $\varphi$ over $\call(\Gamma)$ one can construct a local-LTL formula $\bar \varphi$ 
over $\calh(\Gamma)$
such that for every $u \in \call(\Gamma)$, $u \models \varphi$ iff $h(u) \models \bar \varphi$
where $h((\kappa,stg,\sigma)) = (\kappa, \sigma)$. 
\end{lemma}

\begin{proof}
We use the equivalence of FO and LTL over $\omega$-words. It is easy to see that each LTL formula $\varphi$ 
over $\call(\Gamma)$ can be translated into an FO formula $\psi(\varphi)$ over 
$\calh(\Gamma)$ using only propositions in P$\Sigma$, such that for every $u \in \call(\Gamma)$,
$u \models \varphi$ iff $h(u) \models \psi(\varphi)$. Indeed, it is straightforward to define by FO means 
the stage of each transaction in a given configuration, as well as each proposition in $P \cup \Sigma$ 
in terms of propositions in P$\Sigma$, on words in $\calh(\Gamma)$.  
One can then construct from the FO sentence $\psi(\varphi)$ an LTL formula $\bar \varphi$ 
equivalent to it over words in $\calh(\Gamma)$, using the same set of propositions P$\Sigma$.
The resulting LTL formula is thus in local-LTL.
\end{proof}

We use a propositional variant HLTL of HLTL-FO, 
defined over $\omega$-words in $\calh(\Gamma)$
similarly to HLTL-FO.
More precisely, LTL formulas applying to transaction $T$ use propositions
in $P_T \cup \Sigma^{obs}_T$ and expressions $[\psi]_{T_c}$ where $T_c$ is a child of $T$ and $\psi$ is an HLTL formula applying to 
$T_c$. 

We show the following key fact.


\begin{lemma} \label{lem:hltl}
For each LTL formula over $\calh(\Gamma)$ invariant with respect to interleavings there exists
an equivalent HLTL formula over $\calh(\Gamma)$. 
\end{lemma}

\begin{proof}
By Lemma \ref{lem:local-ltl}, we can assume the LTL formula is in local-LTL. 
To show completeness of HLTL, we use a logic shown in \cite{Gastin-latin, Gastin-infcomp} 
to be complete for expressing LTL properties invariant with respect to interleavings
(or equivalently, well-defined on Marzurkievicz traces).
The logic operates on partial orders $\preceq_u$ 
of words $u \in \calh(\Gamma)$.
We adapt the logic to our framework, and denote it LTL$(\preceq)$. 
For $u = \{(\kappa_i, \sigma_i) \mid i \geq 0\}$, we define the projection of $u$ on $T$ as the 
subsequence $\pi_T(u) = \{(\kappa_{i_j}|_{P_T}, \sigma_{i_j})\}_{j \geq 0}$ where $\{\sigma_{i_j} \mid j \geq 0\}$ 
is the subsequence of $\{\sigma_i \mid i \geq 0\}$ retaining all services in $\Sigma^+_T$.
LTL$(\preceq)$ uses the set of propositions P$\Sigma$ and
the following temporal operators on $\preceq_u$:
\begin{itemize}
\item {\bf X}$_T \varphi$, which holds in $(\kappa_i,\sigma_i)$ if 
$\pi_T(v) \neq \epsilon$ 
for $v = \{(\kappa_j, \sigma_j) \mid j \geq m\}$, where $m$ is the minimum index such that $i \prec_u m$,
and $\varphi$ holds on  $\pi_T(v)$;
\item $\varphi$ {\bf U}$_T$ $\psi$, which holds in $(\kappa_i,\sigma_i)$ if 
$\pi_T(v) \neq \epsilon$ 
for $v = \{(\kappa_j, \sigma_j) \mid j \geq i\}$, and $\varphi$ {\bf U} $\psi$ holds
on $\pi_T(v)$.
\end{itemize}
From Theorem 18 in \cite{Gastin-latin} and Proposition 2 and Corollary 26 in \cite{Gastin-infcomp} it follows that 
LTL$(\preceq)$ expresses all local-LTL properties over $\calh(\Gamma)$ invariant under interleavings 

We next show that HLTL can simulate LTL$(\preceq)$.
To this end, we consider an extension of HLTL in which LTL$(\preceq)$ formulas may be used in addition to
propositions in $P_T \cup \Sigma^+_T$ in every formula applying to transaction $T$. 
We denote the extension by HLTL+LTL$(\preceq)$. Note that for each formula $\xi$ in LTL$(\preceq)$, $[\xi]_{T_1}$ is 
an HLTL+LTL$(\preceq)$ formula. The proof consists in showing that the  LTL$(\preceq)$ formulas can be
eliminated from HLTL+LTL$(\preceq)$ formulas. This is done by recursively reducing the depth of nesting
of $X_T$ and $U_T$ operators, and finally eliminating propositions. 
We define the {\em rank} of an LTL$(\preceq)$ formula to be the maximum number of $X_T$ and $U_T$ operators 
along a path in its syntax tree. For a formula $\xi$ in HLTL+LTL$(\preceq)$, we define $r(\xi) = (n,m)$ 
where $n$ is the maximum rank of an LTL$(\preceq)$ formula occurring in $\xi$, and $m$ is the number of
such formulas with rank $n$. The pairs $(n,m)$ are ordered lexicographically.
 
Let $[\xi]_{T_1}$ be an HLTL+LTL$(\preceq)$ formula. We associate to $[\xi]_{T_1}$ the tree $\T(\xi)$ whose nodes
are all occurrences of subformulas of the form $[\psi]_T$, with an edge 
from $[\psi_i]_{T_i}$ to 
$[\psi_j]_{T_j}$ if the latter occurs in $\psi_i$ and $T_j$ is a child of $T_i$ in $\calh$.

Consider an  HLTL+LTL$(\preceq)$ formula $[\xi]_{T_1}$ such that $r(\xi) \geq (1,1)$. 
Suppose $\xi$ has a subformula ${\bf X}_T \varphi$ in LTL$(\preceq)$ of maximum rank.
Pick one such occurrence and let $\bar T$ be the minimum task (wrt $\calh$) such that ${\bf X}_T \varphi$ occurs in $[\psi]_{\bar T}$.
We construct an HLTL+LTL$(\preceq)$ formula $\bar \xi$ such that $r(\bar \xi) < r(\xi)$, essentially by eliminating
{\bf X}$_T$.  We consider 4 cases: $T = \bar T$, $T$ is a descendant or ancestor of $\bar T$, or neither.

Suppose first that $T = \bar T$. Consider an occurrence of ${\bf X}_T \varphi$. Intuitively, there are two cases: ${\bf X}_T \varphi$ is
evaluated inside the run of $T$ corresponding to  $[\psi]_T$, or at the last configuration. 
In the first case ($\neg \sigma^c_T$ holds),  
${\bf X}_T \varphi$ is equivalent to ${\bf X} \varphi$.
In the second case ($\sigma^c_T$ holds), ${\bf X}_T \varphi$ holds iff $\varphi$ holds at the next call to $T$. Thus, 
$\xi$ is equivalent to $\xi_1 \vee \xi_2$, where: 
\begin{enumerate}
\item $\xi_1$ says that $\varphi$ does not hold at the next call to $T$ (or no such call exists) and 
${\bf X}_T \varphi$ is replaced in $\psi$
by $\neg \sigma^c_T \wedge {\bf X} \varphi$ 
\item $\xi_2$ says that $\varphi$ holds at the next call to $T$ (which exists) and 
${\bf X}_T \varphi$ is replaced in $\psi$
by $\neg \sigma^c_T \rightarrow {\bf X} \varphi$.
\end{enumerate} 
We next describe how $\xi_1$ states that $\varphi$ does not hold at the next call to $T$
($\xi_2$ is similar). We need to state that either 
there is no future call to $T$, or such a call exists and $\neg \varphi$ holds at the first such call. 
Consider the path from $T_1$ to $T$ in $\calh$. Assume for simplicity that the path is
$T_1, T_2, \ldots, T_k$ where $T_k = T$. For each $i$, $1 \leq i < k$, we define inductively (from $k-1$ to $1$)
formulas $\alpha_i, \beta_i(\neg \varphi)$
such that $\alpha_i$ says that there is no call leading to $T$ in the remainder of the current subrun of $T_i$,
and $\beta_i(\neg \varphi)$ says that such a call exists and the first call leads to a subrun of $T$ satisfying $\neg \varphi$.  
First, $\alpha_{k-1} = {\bf G} (\neg \sigma^o_{T_k})$
and $\beta_{k-1}(\neg \varphi) = \neg \sigma^o_{T_k} ~{\bf U} ~[\neg \varphi]_{T_k}$.
For $1 \leq i < k-1$, $\alpha_i = {\bf G} (\sigma^o_{T_{i+1}} \rightarrow [\alpha_{i+1}]_{T_{i+1}})$
and $\beta_i(\neg \varphi) = (\sigma^0_{T_{i+1}} \rightarrow [\alpha_{i+1}]_{T_{i+1}})~{\bf U}~[\beta_{i+1}(\neg \varphi)]_{T_{i+1}}$.
Now $\xi_1 = \xi_1^0 \vee \bigvee_{1 \leq j < k} \xi_1^j$ where $\xi_1^0$ states that there is no next call to $T$
and $\xi_1^j$ states that $T_j$ is the minimum task such that the next call to $T$ occurs during the {\em same} run of $T_j$
(and satisfies $\neg \varphi$).
More precisely, let $[\psi_1]_{T_1}, [\psi_2]_{T_2}, \ldots [\psi_k]_{T_k}$ be the path leading from $[\xi]_{T_1}$
to $[\psi]_{T}$ in $\T(\xi)$ (so $\psi_1 = \xi$ and $\psi_k = \psi$). Then $\xi_1^0$ is obtained by replacing each
$\psi_i$ by $\bar \psi_i$, $1 \leq i < k$, defined inductively as follows. First, $\bar \psi_{k-1}$ 
is obtained from $\psi_{k-1}$ by replacing 
$[\psi_k]_{T_k}$ with $[\psi_k]_{T_k} \wedge \alpha_{k-1}$. For $1 \leq i < k-1$,
$\bar \psi_i$ is obtained from $\psi_i$ by replacing $[\psi_{i+1}]_{T_{i+1}}$ with
$[\bar \psi_{i+1}]_{T_{i+1}} \wedge \alpha_i$. 
For $1 \leq j < k$, $\xi_1^j$ is obtained by replacing in $\psi_j$, $[\psi_{j+1}]_{T_{j+1}}$ with 
$[\bar \psi_{j+1}]_{T_{j+1}} \wedge \beta_j(\neg \varphi)$. 
It is clear that $\xi_1$ states the desired property. The formula $\xi_2$ is constructed similarly.
Note that $r(\xi_1 \vee \xi_2) < r(\xi)$.

Now suppose $T$ is an ancestor of $\bar T$.  We reduce this case to the previous ($T = \bar T$).
Let $T'$ be the child of $T$.  Suppose $[\psi_T]_T$ is the ancestor of 
$[\psi]_{\bar T}$ in $\T(\xi)$.
Then $\xi$ is equivalent to $\bar \xi = \xi_1 \vee \xi_2$ where:
\begin{enumerate}
\item $\xi_1$ says that $\varphi$ does not hold at the next action of $T$ wrt $\preceq$ (or no such next action exists) and
$\psi$ is replaced by $\psi({\bf X}_T \varphi \leftarrow \emph{false})$
\item $\xi_2$ says that $\varphi$ holds at the next action of $T$ wrt $\preceq$ and
$\psi$ is replaced by $\psi({\bf X}_T \varphi \leftarrow \emph{true})$
\end{enumerate}
To state that $\varphi$ does not hold at the next call to $T$ (or no such call exists) 
$\xi_1$ is further modified by replacing in $\psi_T$, $[\psi_{T'}]_{T'}$ with
$[\psi_{T'}]_{T'} \wedge ({\bf G}(\neg \sigma^c_{T'}) \vee (\neg \sigma^c_{T'} ~{\bf U}~ (\sigma^c_{T'} \wedge \neg {\bf X}_T \varphi))$. 
Smilarly, $\xi_2$ is further modified by replacing in $\psi_T$, $[\psi_{T'}]_{T'}$ with
$[\psi_{T'}]_{T'} \wedge (\neg \sigma^c_{T'} ~{\bf U}~ (\sigma^c_{T'} \wedge {\bf X}_T \varphi))$.
Note that there are now two occurrences of ${\bf X}_T \varphi$ in the modified $\psi_T$'s.
By applying twice the construction for the case $\bar T = T$ we obtain an equivalent $\bar \xi$ such that
$r(\bar \xi) < r(\xi)$. 

Next consider the case when $\bar T$ is an ancestor of $T$. Suppose the path from $T_1$ to $T$ in $\calh$
is $T_1, \ldots, T_i, \ldots T_k$ where $T_i = \bar T$ and $T_k = T$.
Consider the value of ${\bf X}_T \varphi$ in the run $\rho_\psi$ of $\bar T$ on which $\psi$ is evaluated.
Similarly to the case $T = \bar T$, there are two cases: 
$\varphi$ holds at the next invocation of $T$ following $\rho_\psi$, or it does not.
Thus, $\xi$ is equivalent to $\xi_1 \vee \xi_2$, where:
\begin{enumerate}
\item $\xi_1$ says that $\varphi$ does not hold at the next call to $T$ (or no such call exists) and
${\bf X}_T \varphi$ is replaced in $\psi$
by $\beta_i(\varphi)$, where $\beta_i(\varphi)$ says that there exists a future call leading to $T$ in the current run of $\bar T$, and 
the first such run of $T$ satisfies $\varphi$; $\beta_i(\varphi)$ is constructed as in the case $T = \bar T$.
\item $\xi_2$ says that $\varphi$ holds at the next call to $T$ following the current run of $\bar T$ and
${\bf X}_T \varphi$ is replaced in $\psi$
by $\alpha_i \vee \beta_i(\varphi)$ where $\alpha_i$, constructed as for the case $T = \bar T$, 
says that there is no future call leading to $T$ in the current run of $\bar T$.
\end{enumerate}
To say that $\varphi$ does not hold at the next call to $T$ following $\rho_\psi$ (or no such call exists), $\xi_1$ is modified analogously to 
the case $\bar T = T$, and similarly for $\xi_2$.

Finally suppose the least common ancestor of $\bar T$ and $T$ is $\hat T$ distinct from both.
Let $[\psi_{\hat T}]_{\hat T}$ be the ancestor of $[\psi]_{\bar T}$ in $\T(\xi)$.
Consider the value of ${\bf X}_T \varphi$ in the run of $\bar T$ on which $\psi$ is evaluated.
There are two cases: $\varphi$ holds at the next invocation of $T$ following the run of $\bar T$, or it does not.
Thus, $\xi$ is equivalent to $\xi_1 \vee \xi_2$, where:
\begin{enumerate}
\item $\xi_1$ says that $\varphi$ does not hold at the next call to $T$ (or no such call exists) and
$\psi$ is replaced by $\psi({\bf X}_T \varphi \leftarrow \emph{false})$
\item $\xi_2$ says that $\varphi$ holds at the next call to $T$ and
$\psi$ is replaced by $\psi({\bf X}_T \varphi \leftarrow \emph{true})$
\end{enumerate}
To say that $\varphi$ does not hold at the next call to $T$ (or no such call exists), $\xi_1$ is modified analogously to
the case $\bar T = T$, and similarly for $\xi_2$, taking into account the fact that the next call to $T$, if it exists,
must take place in the current run of $\hat T$ or of one of its ancestors.
This completes the smulation of {\bf X}$_T \varphi$.

Now  suppose $\xi$ has a subformula $(\varphi_1 ~{\bf U}_T~ \varphi_2)$ of maximum rank.
Pick one such occurrence and let $\bar T$ be the minimum task (wrt $\calh$) such that 
$(\varphi_1 ~{\bf U}_T~ \varphi_2)$  occurs in $[\psi]_{\bar T}$. There are several cases: $\bar T = T$, 
$\bar T$ is an ancestor or descendant of $T$, or neither. The simulation technique is similar to the above.
We outline the construction for the most interesting case when $T = \bar T$.

Consider the run of $T$ on which $[\psi]_T$ is evaluated. There are two cases: 
$(\dag)$ $(\varphi_1 ~{\bf U}_T~ \varphi_2)$ holds on the concatenation of the future runs of $T$, or $(\dag)$ does not hold.
Thus, $\xi$ is equivalent to $\xi_1 \vee \xi_2$ where:

\begin{enumerate}
\item $\xi_1$ says that $(\dag)$ holds and $\psi$ is modified by replacing the occurrence of  $(\varphi_1 ~{\bf U}_T~ \varphi_2)$
with ${\bf G} \varphi_1  \vee ~(\varphi_1 ~{\bf U}~ \varphi_2)$, and

\item $\xi_2$ says that $(\dag)$ does not hold and $\psi$ is modified by replacing the occurrence of  $(\varphi_1 ~{\bf U}_T~ \varphi_2)$
with $(\varphi_1 ~{\bf U}~ \varphi_2)$.
\end{enumerate}

We show how $\xi_1$ ensures $(\dag)$. Let $T_1, \ldots, T_k$ be the path from root to $T$ in $\calh$. 
For each $i$, $1 \leq i < k$, we define inductively (from $k-1$ to $1$)
formulas $\alpha_i, \beta_i$ as follows. Intuitively, $\alpha_i$ says that all future calls leading to $T$ 
from the current run of $T_i$ must result in runs satisfying {\bf G} $\varphi_1$:
\begin{itemize}
\item $\alpha_{k-1} = {\bf G} (\sigma^0_k \rightarrow [{\bf G}~\varphi_1]_{T_k})$,
\item for $1 \leq i < k-1$, $\alpha_i = {\bf G} (\sigma^o_{i+1} \rightarrow [\alpha_{i+1}]_{T_{i+1}})$
\end{itemize}
The formula $\beta_i$ says that there must be a future call to $T$ in the current run of $T_i$ satisfying $\varphi_1 {\bf U} \varphi_2$
and all prior calls result in runs satisfying ${\bf G} \varphi_1$:
\begin{itemize}
\item $\beta_{k-1} = (\sigma^o_k \rightarrow [{\bf G} \varphi_1]_{T_k}) ~{\bf U}~ [\varphi_1 {\bf U} \varphi_2]_{T_k}$,
\item for $1 \leq i < k-1$, $\beta_i = (\sigma^o_{i+1} \rightarrow [\alpha_{i+1}]_{T_{i+1}}) ~{\bf U}~ [\beta_{i+1}]_{T_{i+1}}$.
\end{itemize}
  
Now $\xi_1$ is $\bigvee_{1 \leq j < k} \xi_j$ where $\xi_j$ 
states that the concatenation of runs resulting from calls to $T$ within the run of $T_j$ 
on which $[\psi_j]_{T_j}$ is evaluated, satisfies $(\varphi_1 ~{\bf U}~ \varphi_2)$.   
More precisely, let $[\psi_1]_{T_1}, \ldots, [\psi_k]_{T_k}$ be the path from $[\xi]_{T_1}$ to $[\psi]_T$ in $\T(\xi)$
(so $\psi_1 = \xi$ and $\psi_k = \psi$). For each $j$ we define $\psi_i^j$, $1 \leq i < k$ as follows:
\begin{itemize}
\item if $j < k-1$, $\psi^j_{k-1}$ is obtained from $\psi_{k-1}$ by replacing $[\psi_k]_{T_k}$ with
$[\psi_k]_{T_k} \wedge \alpha_{k-1}$
\item if $j = k-1$, $\psi^j_{k-1}$ is obtained from $\psi_{k-1}$ by replacing $[\psi_k]_{T_k}$ with
$[\psi_k]_{T_k} \wedge \beta_{k-1}$
\item for $j < i < k-1$, $\psi^j_i$ is obtained from $\psi_i$ by replacing $[\psi^j_{i+1}]_{T_{i+1}}$
with  $[\psi^j_{i+1}]_{T_{i+1}} \wedge \alpha_i$
\item $\psi^j_j$ is obtained from $\psi_j$ by replacing  $[\psi^j_{j+1}]_{T_{j+1}}$ with
$[\psi^j_{j+1}]_{T_{j+1}} \wedge \beta_j$
\item for $1 \leq i <j$, $\psi^j_i$ is obtained from $\psi_i$ by replacing $[\psi_{i+1}]_{T_{i+1}}$
with $[\psi^j_{i+1}]_{T_{i+1}}$.
\end{itemize}
Finally, $\xi_j = [\psi^j_1]_{T_1}$. The formula $\xi_2$ is constructed along similar lines.
This completes the case $(\varphi_1~{\bf U}_T~\varphi_2)$

Consider now the case when the formula of maximum rank is a proposition $(p,\sigma) \in $ P$\Sigma$.
Recall that $p \in P_T$ if $\sigma \in \Sigma_T \cup \{\sigma^o_{T'} \mid T' \in \emph{child}(T)\}$ and
$p \in P_T \cup P_{T'}$ if $\sigma = \sigma^c_{T'}$ where $T' \in \emph{child}(T)$.
Suppose that $p \in P_T$ and $\sigma \in  \Sigma_T \cup \{\sigma^o_{T'} \mid T' \in \emph{child}(T)\}$. 
If $(p,\sigma)$ occurs in $[\psi]_{\bar T}$ for some ${\bar T} \neq T$ 
then $(p,\sigma)$ can be replaced with {\em false}.
If $(p,\sigma)$ occurs in $[\psi]_{T}$ then $(p,\sigma)$ can be replaced with $p \wedge \sigma$.
Now suppose that $\sigma = \sigma^c_{T'}$ for some $T' \in \emph{child}(T)$.  If $(p,\sigma^c_{T'})$ occurs in $[\psi_{T'}]_{T'}$
for some $T' \in  \emph{child}(T)$ and $p \in P_{T'}$ then $(p,\sigma^c_{T'})$ is replaced with $p \wedge \sigma^c_{T'}$.
Similarly if $(p,\sigma^c_{T'})$ occurs in $[\psi_{T}]_{T}$
and $p \in P_{T}$ then $(p,\sigma^c_{T'})$ is replaced with $p \wedge \sigma^c_{T'}$.
Suppose $p \in P_T$ and $(p, \sigma^c_{T'})$ occurs in $[\psi_{T'}]_{T'}$. 
There are two cases:  $(\ddag)$ $p$ holds in the run of $T$ on which $[\psi_T]_T$ is 
evaluated when the run of $T'$
on which  $[\psi_{T'}]_{T'}$ is evaluated returns (if ever), or $(\ddag)$ is false. Thus, $\xi = \xi_1 \vee \xi_2$ where:
\begin{itemize}
\item $\xi_1$ says that $(\ddag)$ holds and $\psi_{T'}$ is replaced by $\psi_{T'}[(p,\sigma^c_{T'}) \leftarrow \sigma^c_{T'}]$,
\item $\xi_2$ says that $(\ddag)$ does not hold and  $\psi_{T'}$ is replaced by $\psi_{T'}[(p,\sigma^c_{T'}) \leftarrow \emph{false}]$
\end{itemize}
In order to say that $(\ddag)$ holds, $[\psi_{T'}]_{T'}$ is replaced in $\psi_T$ by
$[\psi_{T'}]_{T'} \wedge [{\bf G}(\neg  \sigma^c_{T'}) \vee (\neg \sigma^c_{T'} ~{\bf U} ~ (p \wedge \sigma^c_{T'}))]$.
To say that $(\ddag)$ does not hold, $[\psi_{T'}]_{T'}$ is replaced by
$[\psi_{T'}]_{T'} \wedge (\neg \sigma^c_{T'} ~{\bf U} ~ (\neg p \wedge \sigma^c_{T'}))$.

Now suppose that $(p, \sigma^c_{T'})$ occurs in $[\psi_T]_T$ and $p \in P_{T'}$.
To express $(p,\sigma^c_{T'})$ we use the past temporal operator {\em since} denoted {\bf S},
whose semantics is symmetric to {\bf U} \cite{}.
It is known that past temporal operators can be simulated in LTL \cite{}.
The occurrence of $(p,\sigma^c_{T'})$ is replaced in $\psi_T$ by the formula
$\sigma_{T'}^c \wedge ((\neg \sigma^o_{T'})~{\bf S}~ [{\bf F}(\sigma^c_{T'} \wedge p)]_{T'})$.

This concludes the proof of the lemma.
\end{proof}

Theorem \ref{thm:complete} now follows. Let $\varphi_f$ be an LTL-FO formula over $\Gamma$, 
invariant under interleavings. By Lemma \ref{lem:local-ltl}, we can assume that $\varphi$ is in local-LTL
and in particular uses the set of propositions P$\Sigma$. 
By Lemma \ref{lem:hltl}, there exists an HLTL formula $[\xi]_{T_1}$ equivalent to $\varphi$ over $\omega$-words in 
$\calh(\Gamma)$, using propositions
in $P \cup \Sigma$. 
Moreover, by construction, each sub-formula $[\psi]_T$ of $[\xi]_{T_1}$ uses only propositions
in $P_T \cup \Sigma^+_T$. 
It is easily seen that formula obtained by replacing each $p$ with $f(p)$ is a well-formed HLTL-FO formula
equivalent to $\varphi_f$ on all runs of $\Gamma$.
 




